Analysis and Design of Thompson Sampling for Stochastic Partial Monitoring

We investigate finite stochastic partial monitoring, which is a general model for sequential learning with limited feedback. While Thompson sampling is one of the most promising algorithms on a variety of online decision-making problems, its properties for stochastic partial monitoring have not been theoretically investigated, and the existing algorithm relies on a heuristic approximation of the posterior distribution. To mitigate these problems, we present a novel Thompson-sampling-based algorithm, which enables us to exactly sample the target parameter from the posterior distribution. Besides, we prove that the new algorithm achieves the logarithmic problem-dependent expected pseudo-regret $\mathrm{O}(\log T)$ for a linearized variant of the problem with local observability. This result is the first regret bound of Thompson sampling for partial monitoring, which also becomes the first logarithmic regret bound of Thompson sampling for linear bandits.

==> tex_src/practical_implementation.tex <==
\section{Practical Implementation}
\label{sec:practical}
With Theorem~\ref{thm:ssl-cvx-surrogate-risk}, we can obtain a risk estimator that can fully use both labeled and unlabeled data. It is straightforward to see that our risk estimator based on Theorem~\ref{thm:ssl-cvx-surrogate-risk} is unbiased. However, to use our risk estimator effectively, one important question is: \emph{how can we decide the class $k$ to calculate $\empRluk(g)$?}
We discuss strategies to handle this problem theoretically.

\subsection{Strategies to Remove One Class for $\empRluk(g)$}
\label{subsec:what-class-to-pick-out}
We discuss some guidelines to select a class to remove for $\empRluk(g)$.
We provide two strategies.

The first strategy is based on finite sample estimation error.
More specifically, when we approximate the expectation
term by a limited number of samples, the variance of the estimator can be large.
Then a naive strategy would be to remove the class that contains the smallest number of labeled data:
\begin{equation}
    \label{eq:strategy1}
    k = \argmin_{y\in \mathcal{Y}} n_y.
\end{equation}

The other strategy is based on the estimation error bound.
As discussed in Theorem~\ref{thm:estimation-error-bound}, the convergence rate of the estimation error is
$\mathcal{O}_p(\sum_{y\in\calYrmk} {\pi_y}/{\sqrt{n_y}} + 1/\sqrt{n_\u})$, where $\mathcal{O}_p$ denotes the order in probability.
This implies the following proposition which provides a strategy to decide the removed class $k$:
\begin{proposition}
\label{cor:what-class-to-pick-out-joint}
  If labeled data are obtained under the assumption in Eq.~\eqref{eq:joint-assumption},
  $k \in \mathcal{Y}$ such that
  \begin{align}
      \label{eq:strategy2}
      k &= \argmax_{y\in \mathcal{Y}} {n_y}
  \end{align}
  gives the lowest upper bound of the estimation error.
\end{proposition}
It is interesting to see that the above two strategies give completely opposite solutions. We will experimentally compare these strategies in Section~\ref{sec:experiments}.



\subsection{Order Constraints}\label{sec:thr-con}
In ordinal regression problems, the threshold parameters should be ordered, \ie $\theta_1 \leq \theta_2 \leq \cdots \leq \theta_{K-1}$~\citep{pedregosa:consistency}.
Here, we introduce a simple trick to constrain the threshold parameters $\btheta$ by adding the following term:
\begin{align}
\label{eq:order-constraints}
  \Omega(\btheta) \coloneqq \mu \cdot \max \left\{0,\ \sum_{i=1}^{K-2} -\log (\theta_{i+1} - \theta_i) \right\},
\end{align}
where $\mu \geq 0$ is a regularization parameter for the order constraints.
We show that this simple trick works well in the experiments.
In fact, even without any regularization term on $\btheta$,
we empirically observed that the values of threshold constraints $\btheta$ are usually ordered.
This observation suggests that the order constraints are not difficult to satisfy for the solution of the optimization problem.
This threshold regularization scheme is based on the idea of the log-barrier method~\citep{boyd2004convex},
in which we impose a high cost to the objective function when $\theta_{i+1} - \theta_i\ (i=1,\ldots,K-2)$ are close to $0$.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.67\columnwidth]{fig/loss_arxiv.pdf}
    \caption{Examples of the binary surrogate losses satisfying Eq.~\eqref{eq:margin-loss-cond}.}
    \label{fig:binary-surr}
\end{figure}

\begin{table}[t]
    \centering
    \caption{Binary surrogate losses that can be used for binary classification and their satisfiability of the sufficient condition in Eq.~\eqref{eq:margin-loss-cond}.}
    \label{tab:binary-surr}
    \begin{tabular}{CCC  C  C  C  C}
        \hline
        \text{Loss name} & \ell(z)  & \text{Eq.~\eqref{eq:margin-loss-cond}}\\ \hline
        %\text{Ramp} & -0.5 \max(0, \min(1, 0.5-0.5z)) &\times\\
        \text{Hinge} & \max(0, 1-z)  & \text{No} \\
        \text{Exponential} & \exp(-z) & \text{No} \\
        %\text{Sigmoid} & \left[1+\exp(z)\right]^{-1} &\times\\
        \text{Logistic} & \log(1+e^{-z}) & \text{Yes} \\
        \text{Double-hinge} & \max(-z, \max(0, \frac{1}{2} - \frac{1}{2}z)) & \text{Yes} \\
        \text{Squared} & (1-z)^{2}  & \text{Yes} \\ \hline
        %\text{Perceptron} & \max(-z,0) &\checkmark
    \end{tabular}
\end{table}


Here, we investigate the objective function when the linear-in-parameter model
$f(\x) = \bw^\top \bphi(\x)$ is employed as $f$,
where $\bw \in \R^b$ is a parameter and
$\bphi: \R^d \rightarrow \R^b$ is a basis function.
We assume that the bias parameter is included in $\bw$.
Then, our next theorem states a sufficient condition to guarantee that, for a certain task surrogate loss function, the optimization problem is convex with respect to both the model and order constrains parameters.%~\eqref{eq:optimization-problem}.
\begin{theorem}
  \label{thm:convex-ssl-or}
  Let $C_\ell$ be a positive constant.
  If the AT loss $\psi_\AT (\balpha, y)$ is adopted as the task surrogate loss,
  and the binary surrogate loss $\ell(z)$ is convex and satisfies
  \begin{align}
    \ell(z) - \ell(-z) = -C_\ell z
    \label{eq:margin-loss-cond}
    ,
  \end{align}
  then the objective function $\hat{J}_\ell(\bw, \btheta) \coloneqq \calR_{\psi,\SEMI\text{-}\gamma}^{\backslash k}(g) + \Omega(\btheta)$ is convex with respect to $\bw$ and $\btheta$.
\end{theorem}
\allowdisplaybreaks
The proof of Theorem~\ref{thm:convex-ssl-or} is given in Appendix~\ref{sec:proof-of-convex-ssl-or}.
Also, if the least-squares or least absolute deviation loss is adopted as the task surrogate loss,
then $\hat{J}_\ell(\bw, \btheta)$ is convex with respect to the parameter $\bw$ and $\btheta$
(details of the least absolute deviation and least-squares losses are shown in Appendix~\ref{sec:proof-of-convex-ssl-or} and the work by~\citet{pedregosa:consistency}).
The condition in Eq.~\eqref{eq:margin-loss-cond} is known as the linear-odd condition~\citep{patrini2016loss}.
% ,
%which has been considered in many weakly-supervised learning problems
%such as learning from positive-unlabeled data~\citep{du2015convex} and learning from pairwise and similarity data~\citep{baosu}.
Examples of binary surrogate losses are shown in Figure~\ref{fig:binary-surr} and Table~\ref{tab:binary-surr}.
In our experiments, we used the logistic loss as the binary surrogate loss.

\subsection{Non-Negative Risk Estimator}
\label{subsec:nn-risk}
We discuss a risk modification technique called a \emph{non-negative risk estimator}.
This technique was orignally proposed by~\citet{kiryoNNPU2017} for classification from positive and unlabeled data based on an unbiased risk estimator.
We can see that the sum of the second and third term of our empirical risk estimator $\empRU(g) - \empRLtwo(g)$ can be negative while the corresponding expected risk $\RU(g) - \RLtwo(g) = \pi_k \expect_{X|Y=k}\left[ \psi(\balpha(X), k) \right]$ is always non-negative.
This observation suggests that it happens that the model tries to reduce the empirical risk by maximizing $\empRLtwo(g)$.
To prevent this problem, following~\citet{kiryoNNPU2017}, we modify the empirical risk estimator as follows:
\begin{align}
  \empRluk(g)
  &\coloneqq \empRLone(g)
  + \max \left\{0,\empRU(g) - \empRLtwo(g) \right\}
  \label{eq:nn-ssl-or-surrogate-estimator}
  .
\end{align}
The practical implementation to minimize the risk~\eqref{eq:nn-ssl-or-surrogate-estimator} is shown in~\citet{kiryoNNPU2017}.


==> tex_src/previous_writing.tex <==
\section{Previous Writing}
\begin{definition}[Cell decomposition and its properties~\citep{Bartok11minimax}]
    For every action $i\in[N]$, let $\calC_i$ be the set of opponent strategies for which action $i$ is optimal.
    Each optimality cell is a convex closed polytope.
    Also, we say action $i$ is
    \emph{dominated} if $\Ci = \emptyset$;
    \emph{degenerate} if its action is non-diminated and there exists an action $j$ such that $\Ci \subsetneq \Cj$;
    \emph{Pareto-optimal} if its action is neigher dominated nor degenerate.
    % \begin{itemize}
    %     \item \emph{dominated} if $\Ci = \emptyset$;
    %     \item \emph{degenerate} if its action is non-diminated and there exists an action $j$ such that $\Ci \subsetneq \Cj$;
    %     \item \emph{Pareto-optimal} if its action is neigher dominated nor degenerate.
    % \end{itemize}
    \todo{say (maybe) just consider Pareto-optinal sub-opbimal arm.}
\end{definition}


\begin{definition}[Neighbors~\citep{Bartok11minimax}]
    Two Pareto-optimal actions $i$ and $j$ are~\emph{neighbors} if $\Ci \cup \Cj$ is an $(M-2)$-diensional polytope.
    Also, we define
\end{definition}


\begin{proposition}
    $M \geq 2$を仮定する。
    \blue{（次の仮定一般性を失うがOK...?）loss matrix で同一の行が存在するならば、その feedback　も同じであるような PM game のみを考える。}
    このとき、$\Ci, \Cj$が$(M-1)$次元以上($(M-2)$次元より大きい)であるような任意の$i,j\in[N]$に対して、$\Nplus{i}{j} = \ev{i, j}$である。
    すなわち、
    \begin{align}
        \left[S_i^\top S_j^\top \right] z = L_i - L_j
    \end{align}
    （すなわち、青い本のrankの形で書ける）。
    \ask{loss matrix の行が同じで、feedbackが異なるような設定を考えると、local observability condition を考えるときに、$\Nplus{i}{j} = \ev{i, j}$ とはならず厳しい。}
\end{proposition}
\begin{proof}
    loss matrix で同一の行が存在するならば、その feedback　も同じであるような PM game のみを考えているが、
    もしそのような行が存在すれば、同一のものだとみなす（同一のアクションだとみなして一般性を失わない）。
    今、$\Ci$が$(M-1)$次元（$(M-2)$次元より大きい次元を持つ）であるような、$i\in[N]$を考える。
    このとき、$i$がdominatedであると仮定すると次元が$0$であることから$M>2$より、 $i$はnon-diminated。
    また、not degenerate (何故ならば denerate していると仮定するとそのような cell は $(M-2)$次元以下。
    \todo{本当か怪しいが、直感的には細胞分割したときに $(M-2)$次元のあるセルが、$(M-2)$次元の別のアクションのセルの真部分集合となることはない。}
    よって、以上の考察より、
    $\Ci, \Cj$が$(M-1)$次元以上($(M-2)$次元より大きい)任意の$i,j\in[N]$に対して、
    neigborhoood action set の定義より、
    $\Nplus{i}{j}=\ev{i,j}$である。
    \todo{あーこれ嘘です。iPadの写真を見る。写真中の$S_\ell$が不要になる条件について考察する！}
    \ask{そもそもBPMの論文 $\ell_i - \ell_j \in \Img S_i^\top \oplus S_j^\top$  にしとるし...}
    したがって、
    local observability condition は、
    $L_i - L_j \in \oplus_{k \in \ev{i,j}} \Img S_k^\top$,
    すなわち、
    任意の $i, j \in [N]$ に対して、（$i,j$に依存した）ある $z \in \R^{2A}$ が存在して、
    \begin{align}
        \left[S_i^\top S_j^\top \right] z = L_i - L_j
    \end{align}
    が条件であると言える。
    （青い本のrankの形で書ける）。
\end{proof}

